Bounding Fixed Points of Set-Based Bellman Operator and Nash Equilibria of Stochastic Games

Motivated by uncertain parameters encountered in Markov decision processes (MDPs) and stochastic games, we study the effect of parameter uncertainty on Bellman operator-based algorithms under a set-based framework. Specifically, we first consider a family of MDPs where the cost parameters are in a given compact set; we then define a Bellman operator acting on a set of value functions to produce a new set of value functions as the output under all possible variations in the cost parameter. We prove the existence of a fixed point of this set-based Bellman operator by showing that it is contractive on a complete metric space, and explore its relationship with the corresponding family of MDPs and stochastic games. Additionally, we show that given interval set bounded cost parameters, we can form exact bounds on the set of optimal value functions. Finally, we utilize our results to bound the value function trajectory of a player in a stochastic game.

==> IntervalMDP.tex <==
\section{Example}
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.6\columnwidth]{fig/MDP_ex.png}
    \caption{2 state 2 action MDP }
    \label{fig:2S2A_MDP}
\end{figure}
Suppose we have a 2 state, 2 action MDP given by Figure~\ref{fig:2S2A_MDP}, whose cost and transition probabilities are given by Table~\ref{tab:2S2A_P}.
\begin{table}[h]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
& $(1, a_1)$ & $(1, a_2)$ & $(2, a_1)$ & $(2, a_2)$ \\ \midrule
$P_{1, (s,a)}$ & 0.9        & 0.1          & 0.9        & 0.5          \\
$P_{2, (s,a)}$ & 0.1        & 0.9          & 0.1        & 0.5          \\
$C_{s,a}$      & $4 \pm 0.6$          & $5  \pm 0.7$        & $3 \pm 0.5$    & $1 \pm 1$         \\ \bottomrule
\end{tabular}
\label{tab:2S2A_P}
\end{table}
The cost has uncertainty within the given bounds. We investigate using a couple different methods to calculate the value function bounds on this system. I.e. by using interval arithmetic, affine arithmetic, and Sarah's secret sauce arithmetic, apply value iteration and see where it takes me. 

For each of the three methods, we are mostly concerned with addition/subtraction of intervals, multiplication by a scalar, and minimization over a discrete set. 

\subsection{Interval Arithmetic}
Interval arithmetic follows these rules for the different operations. 
\begin{equation}
    \begin{aligned}
        [a, b] + [c, d] & = [a + c, b + d] \\
        [a, b] - [c, d] & = [a - c, b - d] \\
        \min\{[a, b], [c, d]\} &  = [\min\{a, c\}, \min\{b, d\}]
    \end{aligned}
\end{equation}
The cost uncertainties written in interval form is $C_{ii} = [\underline{C_{ii}}, \overline{C_{ii}}]$. 

\subsubsection{Zeroth iteration}
Going through value function iteration, the initial value function is given by
\begin{equation}
    \begin{aligned}
        V_0(1) & = \min\{[\underline{C_{11}}, \overline{C_{11}}], [\underline{C_{12}}, \overline{C_{12}}]\} \\
        V_0(2) & = \min\{[\underline{C_{21}}, \overline{C_{21}}], [\underline{C_{22}}, \overline{C_{22}}],\}
    \end{aligned}
\end{equation}

From interval arithmetics, 
\begin{equation}
    \begin{aligned}
        V_0(1) & = [\min\{\underline{C_{11}}, \underline{C_{12}}\}, \min\{\overline{C_{11}},  \overline{C_{12}}\}] \\
        V_0(2) & = [\min\{\underline{C_{21}}, \underline{C_{22}} \}, \min\{\overline{C_{21}}, \overline{C_{22}}\} ]
    \end{aligned}
\end{equation}

Let $\min\{\underline{C_{s1}}, \underline{C_{s2}}\} = \underline{V_0}(s)$ and  $\min\{\overline{C_{s1}}, \overline{C_{s2}}\} = \overline{V_0}(s)$, then the interval becomes 
\begin{equation}
    \begin{aligned}
        V_0(s) & = [\underline{V_0}(s),\overline{V_0}(s)]
    \end{aligned}
\end{equation}

\subsubsection{First iteration}
The first iteration is 
\[V_1(s)  = \min_{a} C_{sa} + P_{1sa}V_0(1) + P_{2sa}V_0(2),\]
Since each state has two actions, the minimization occurs over 2 distinct elements, i.e.
\[V_1(s) = \min\{ C_{s1} + P_{1s1}V_0(1) + P_{2s1}V_0(2), C_{s2} + P_{1s2}V_0(1) + P_{2s2}V_0(2)\}\]
However now we must treat each element as a set. The first element's interval is represented by 
\[[\underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2)]\]
While the second element is represented by
\[[\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2), \overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)]\]
To obtain the interval representation of $V_1(s)$, which is the minimum over the two intervals given above, we skip a couple steps and get $V_1(s)$ is
\begin{align}
V_1(s) =  [&\min\{ &\underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \\
    &   &\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2)\}, \\
    & \min \{&\overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2), \\
    &   &\overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)\}]
\end{align}
Let
\begin{align}
\underline{V_1}(s) = \min\{& \underline{C_{s1}} + P_{1s1}\underline{V_0}(1) + P_{2s1}\underline{V_0}(2), \\ &\underline{C_{s2}} + P_{1s2}\underline{V_0}(1) + P_{2s2}\underline{V_0}(2)\}
\end{align}
and 
\begin{align}
\overline{V_1}(s) = \min \{&\overline{C_{s1}} + P_{1s1}\overline{V_0}(1) + P_{2s1}\overline{V_0}(2), \\
&\overline{C_{s2}} + P_{1s2}\overline{V_0}(1) + P_{2s2}\overline{V_0}(2)\}
\end{align}

Then $V_1(s) = [\underline{V_1}(s), \overline{V_1}(s)]$ holds.

Here we note that this far, each $\underline{V_i}(s)$ represents the lower bound of the possible value functions given uncertainty in cost function. However, through our derivation, it is obvious they are the results of taking value iteration over constant costs $\underline{C}$ for the lower bounds of the uncertainty in cost. Equivalently, $\overline{V_i}(s)$ represents the upper bound of the possible value functions given uncertainty in cost function; they are also the results of running precise value iteration on the upper bounds $\overline{C}$ of the cost function uncertainty. 

Based on this, the following theorem can be stated ( will prove at some point), 
\begin{theorem}
For an MDP with cost uncertainty given by $C \in [\underline{C}, \overline{C}]$, the value iteration algorithm returns, at the the $k^{th}$ step, a value function $V_k \in [\underline{V_k}, \overline{V_k}]$, where at each state, the upper and lower bounds are given by  
\begin{align}
\overline{V_k}(s) &  = \min_{a} \overline{C_{sa}} + \sum_{s'}P_{s'sa}\overline{V_{k-1}}(s) \\
\underline{V_k}(s) &  = \min_{a} \underline{C_{sa}} + \sum_{s'}P_{s'sa}\underline{V_{k-1}}(s) 
\end{align}
\end{theorem}

This is a fairly general result, it states that even if the costs are \emph{changing}, such that the resulting value iteration does \emph{not} converge, the value functions cannot leave the bounds given by $\underline{V_k}$ and $\overline{V_k}$. 

A natural consideration is, will value iteration also converge to the values given within these bounds? The answer is no. To see this, just consider when we choose $\underline{C} \in [\underline{C}, \overline{C}]$, the element that's the absolute lower bound. Because value iteration always returns an upper bound, we are guaranteed that $\underline{V}^\star \leq \underline{V}_k$ for all $k$. 

However when MDP is ergodic, we do have some sort of bound on $V_k$ for the mean average pay off case. 

==> Proposal.tex <==

\section{Bounding value approximation}
\label{sec:templates}

\ForAuthorsAssa{I will develop this part}
Given an input uncertain cost $\mc{C}$, we can outer approximate the output of $F_{\mc{C}}$ by a given template $h: \reals^S \rightarrow \reals^m$ and a bounding vector $\alpha_v \in \reals^m$ which satisfies 
\[F_{\mc{C}}(\mc{V}) \subseteq \Lambda = \{V \ | \ h(V) \leq \alpha_v\}\]
How closely $h(\mc{V}) \leq \alpha_v$ approximates $F_{\mc{C}}$ depends on both the template $h$ and the bounding vector $\alpha_v$. If the shape of $F_{\mc{C}}$ wildly differs the shape of $h$, then it's impossible to obtain a good approximation of $F_{\mc{C}}$. For the rest of this paper, we assume that $h$ is an \emph{affine function} in $V$, such that its sublevel sets are polytopes. Assuming that the given template $h$ can provide a good approximation, the quality of approximation then depends on $\alpha_v$.
\ForAuthorsAssa{By tight, you mean there is no $\alpha\in\reals^m$ such that $\{V\mid h(V)\leq \min (\alpha,\alpha_v)\}$ contains $F_{\mc{C}}(\mc{V})$?}
\tc{red}{yeah that sounds right}


\begin{proposition}
For each $j \in [m]$, approximating $F_{\mc{C}}(\mc{V})$ by $\Lambda  = \{V \ | \ h(V) \leq \alpha_v\} $ is tight if for each $j \in [m]$, 
\[\alpha_{vj} = \max_{C\in \Gamma, V \in \mc{V}}\  h_j(f_{C}(V))\]
\end{proposition}
\tc{blue}{As we said, we have to maximize on the closed convex hull of $F_{\mc{C}}(\mc{V})$ as $\Lambda$ is closed and convex.}
\begin{proof}
Two things: 1) that $F_{\mc{C}}(\mc{V}) \subseteq \Lambda$. This can be shown with the hyperplane separation theorem. 2) that for any $\alpha < \alpha_v$, the set $\Lambda$ will not contain $F_{\mc{C}}(\mc{V})$. This probably can also be shown with the hyperplane separation theorem. 
\end{proof}

\tc{blue}{I do not understand the proof. The maximizer $V^*$ of $h$ does not satisfy $V\leq V^*$ for all $V\in\mc{V}$. Then $f_C(V^*)$ is not necessarily better than $f_C(V)$ for all $V\in\mc{V}$. For example, take $h(x,y)=x-y$, $\mc{V}=[-10;10]\times [-5,5]$ and $f(x,y)=(\min(x,y),\max(x,y))$. The maximizer $V^*$ of $h$ on $\mc{V}$ is $(10,-5)$. Then $h(f(V^*))=\min(10,-5)-\max(10,-5)=-15$. However $\max_{(x,y)\in \mc{V}} h(f(x,y))\geq h(f(0,0))=0$.}

\tc{blue}{The aim of the theorem is to construct an algorithm to compute a representation of $F_\mc{C}(\mc{V})$ and for a given $h$ how to compute the value $\alpha$. }
\tc{red}{Hi Assale, this proposition should not hold for any general $F$, it should hold for just the bellman operator $F_{\mc{C}}$, which is an order preserving operator. We can talk about it tomorrow. This is basically my understanding of what you wrote on the board when we talked in Toulouse. }
\begin{theorem}
If $F_\mc{C}(\cdot)$ is an order preserving operation, each approximation $\Tilde{\Lambda}$ is determined by its coefficient and can be solved as 
\begin{align}
    \alpha_v &  =  \underset{C \in \Gamma, V\in\mc{V}}{\max } \ h(f_{C}(V))\\
    &  = \max_{C\in \Gamma}h\circ f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big) \\
    % &  = h\circ \max_{C\in \Gamma}f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big) \\
    &  = h\circ f_{C^\star}\Big(V^\star\Big) 
\end{align}
where $V^\star = \argmax_{V\in\mc{V}}h_j(V)$, and $C^\star = \argmax_{C \in\Gamma}h_j(f_{C}(V^\star))$
\end{theorem}
\
\ForAuthorsAssa{In the case where $x\mapsto h(x)=-x_i$, $h$ is not order-preserving. However, $-h$ is order-preserving and then $\max h=-\min -h$ and then we can extend the result to the min and we have $\max h=-F(z,-h(\argmin_{C\in\Gamma} C)$  }
\begin{proof}
Given $V$ and uncertainty set $\Gamma$, the output value functions are defined by 
\[F_{\mc{C}}(\mc{V}) = \{ V^+ \ | \ \exists\ C\in \Gamma, \ V\in \mc{V}, \ \text{ s.t. } V^+ = f_{C}(V)\}\]

We consider using generic template $h$ to over-approximate $F_{\mc{C}}(\mc{V})$. From Proposition 1, 
\[\alpha =  \underset{C \in \Gamma, V \in \mc{V}}{\max }\  h(f_{C}(V)) \]
First, we note that since neither $h$ or $f_{C}$ depends on $V$, and $f_C$ is a order preserving operator over $V$, we can take the maximization over $V$ directly to within $f_C$. 
\[\alpha = h\circ f_{C}\Big(\argmax_{V\in\mc{V}}h(V)\Big)\]
Let $V^\star = \argmax_{V\in\mc{V}}h_j(V)$. Then because $h$ does not involve $C$, we can take the maximization over $\Gamma$ directly in $f_C$.  
Let $C^\star = \argmax_{C \in \Gamma} h_j(f_C(V^\star))$ ,
\[\alpha_j = h_j\Big( f_{C^\star}(V^\star)\Big)\]
\end{proof}




==> samePolicy.tex <==
\section{effects of cost uncertainty on policy}
\tc{red}{This is migrating to another overleaf soon}
Often in MDP related problems, we ask the following question: given a cost $C$, determine the set of optimal policies. However a reverse question can also be interesting: given a policy, what is the set of corresponding costs for which the policy is optimal? This is a more difficult question for two reasons. The first difficulty is determining a single cost for which a given policy is optimal. This is not a well examined problem so far. The second is determining a set of costs around this single cost that still guarantees optimality of the given policy. We show here that this can be addressed by utilizing our problem set up. Formally, the problem we attempt to solve is: given an uncertainty range around a cost for which a policy is optimal, how can we determine if the policy is optimal for the entire set of possible costs? 

\begin{theorem}
Given uncertainty cost interval $[\underline{C}, \overline{C}]$, if a policy $\pi$ is optimal for both the MDP defined by $\underline{C}$ and $\overline{C}$, then it is optimal for all MDP's corresponding to any cost $C\in [\underline{C}, \overline{C}]$. 
\end{theorem}
\begin{proof}
Suppose that $\pi$ is optimal for the MDP's defined for $\underline{C}$ and $\overline{C}$. Then we have that 
\[\underline{V} = (I - \gamma P\pi^T)^{-1}\underline{C},\  \overline{V} = (I - \gamma P\pi^T)^{-1}\overline{C}\]
For an element $C \in [\underline{C}, \overline{C}]$, we have that the corresponding optimal value function satisfies
\[ V = \min_{\pi \in \Pi} (I - P\pi^T)^{-1}C\pi^T \]
First we note that taking the minimum of a finite number of convex functions is a convex operation.\tc{red}{Is this $(I - P\pi^T)^{-1}C\pi^T$ convex?? yes it is, taking $C$ as the variable} 
Let the operation be defined by $p(C)$. Since $C_{s\pi(s)} \in [\underline{C}_{s\pi(s)}, \overline{C}_{s\pi(s)}]$, we have that 
\begin{align}
f(C) &\geq (1 - \lambda)f(\overline{C}) + \lambda f(\underline{C}) \\
& \geq (1 - \lambda)(I - \gamma P\pi^T)^{-1}\overline{C}\pi^T + \lambda (I - \gamma P\pi^T)^{-1}\underline{C}\pi^T \\
\min_{\pi \in \Pi} (I - \gamma P\pi^T)^{-1}C\pi^T & \geq (I - \gamma P\pi^T)^{-1}((1 - \lambda)\overline{C} + \lambda \underline{C})\pi^T \\
\min_{\pi \in \Pi} (I - \gamma P\pi^T)^{-1}C\pi^T & \geq (I - \gamma P\pi^T)^{-1}C\pi^T
\end{align}
Therefore, we see that $\pi$ minimizes the set of possible stationary value functions. We conclude that $\pi$ is optimal for any cost function $C \in [\underline{C}, \overline{C}]$ 

\end{proof}

==> summary.tex <==
\newpage
\appendix
\section{Summary}
current structure
\begin{enumerate}
    \item[3] MDP and Bellman op
    \begin{enumerate}
        \item[] def of MDP, policy
        \item[] discounted infinite horizon expected cost
        \item[A] Bellman operator
        \begin{enumerate}
            \item[] Bellman op 
            \item[] \textbf{Def 1} : Fixpoint
            \item[] \textbf{Thm1}: existence of the fixpoint 
        \end{enumerate}
        \item[B] Termination criteria for value iteration
        \begin{enumerate}
            \item[] \textbf{Thm 2}: convergence of VI
        \end{enumerate}
    \end{enumerate}
    
    \item[4] Set-based value iteration
    \begin{enumerate}
    \item[] Haussdorf distance btw sets
    \item[] \textbf{Thm3} Haussdorf metric space of a complete metric space (cms) is a cms
    \item[] \textbf{Prop1}: when C compact, $F_C(V)$ in the same cms as V
    \item[] \textbf{Def2} Lower/Upper semi-continuous func
    \item[] \textbf{Lemma 1}: inf+closure on lower semi-cont. func
    \item[] \textbf{Lemma 2}: sup-inf + closure
    \item [] \textbf{Prop2}: $F_C$ is order preserving+contracting
    \item [] \textbf{Def3}: order preserving
    \item[] \textbf{Def4}: contracting
    \item [] \textbf{Prop 3}: banach fixpoint thm on cms
    \item [] \textbf{Def5}: set-based fixpoint (and $\bar{V}$)
    \item[A] Bounding value approx
        \begin{enumerate}
            \item[] template abstraction
            \item[] \textbf{Prop4}: tight abstraction
            \item[] \textbf{Thm4}: characterization of template bounds on order preserving functions
            \item[] \textbf{Example 1}: interval templates
            \item [] \textbf{Corollary 1}: ??? don't understand what it means
        \end{enumerate}
    \end{enumerate}
    \item[5] Bounding values on stochastic game
    \begin{enumerate}
        \item[A] Stochastic game
        \item[B] Grid MDP
        \item[C] Algorithms
        
    \end{enumerate}
\end{enumerate}
\newpage 
~\\
proposed structure
\begin{enumerate}
    \item[3] MDP and Bellman op\\
    BASIC DEFINITIONS: NO MENTION OF SETS YET
    \begin{enumerate}
        \item[A] MDP and optimal value
        \begin{enumerate}
        \item[] \textbf{Def}: def of MDP, policy
        \item[] \textbf{Def}: discounted infinite horizon expected cost
        \end{enumerate}
        \item[B] Bellman operator fixpoint: optimal value
        \begin{enumerate}
            \item[] \textbf{Def}: Bellman op 
            \item[] \textbf{Def 1} : Fixpoint
            \item[] \textbf{Thm1}: existence of the fixpoint 
        \end{enumerate}
        \item[C] Effective computation using value iteration, Termination criteria
        \begin{enumerate}
            \item[] \textbf{Thm 2}: convergence of VI
        \end{enumerate}
    \end{enumerate}
    
    \item[4] Set-based value iteration\\
    HERE WE DEFINE THE EXTENSION TO SETS AND ARGUE ABOUT THE EXISTENCE OF THE FIXPOINT OF THE LIFT OF BELMANN TO SETS
    \begin{enumerate}
    \item[] \textbf{Def}: Haussdorf distance btw sets
    \item[] \textbf{Thm3} Haussdorf metric space of a complete metric space (cms) is a cms
    \item[] \textbf{Prop1}: when C compact, $F_C(V)$ in the same cms as V
    \item[] \textbf{Def2} Lower/Upper semi-continuous func
    \item[] \textbf{Lemma 1}: inf+closure on lower semi-cont. func
    \item[] \textbf{Lemma 2}: sup-inf + closure
    \item [] \textbf{Def3}: order preserving
    \item[] \textbf{Def4}: contracting
    \item [] \textbf{Prop2}: $F_C$ is order preserving+contracting
    \item [] \textbf{Prop 3}: banach fixpoint thm on cms
    \item [] \textbf{Def5}: set-based fixpoint (and $\bar{V}$)
    \end{enumerate}
    
    \item[5] Template-based abstraction of set-based value iteration\\
    TODO: REDEFINE THE SET EXTENSION OF MDP WITH THE FUNCTION g(C) AND THE TEMPLATE h
        \begin{enumerate}
            \item[] \textbf{Def}: template abstraction, introduce the bounds more formally. 
            \item[] \textbf{Prop4}: tight abstraction
            \item[] \textbf{Thm4}: characterization of template bounds on order preserving functions\\
            here $\tilde{\Lambda}$ is mentioned but never used, you implicitly assume it is related to $\alpha_v$ 
        \end{enumerate}
    \item[6] Example\\
    COULD YOU PROVIDE TWO INSTANCIATIONS FOR h, ONE WITH INTERVAL TEMPLATES AND ONE WITH ANOTHER LINEAR RELATIONSHIP OR A QUADRATIC ONE?
    \begin{enumerate}
                \item[] \textbf{Example 1}: interval templates
            \item [] \textbf{Corollary 1}: ??? don't understand what it means
    \end{enumerate}

    \item[7] Bounding values on stochastic game
    \begin{enumerate}
        \item[A] Stochastic game
        \item[B] Grid MDP
        \item[C] Algorithms
        
    \end{enumerate}
    \end{enumerate}
    
